Calibration Using Matrix Completion with Application to Ultrasound Tomography

We study the calibration process in circular ultrasound tomography devices where the sensor positions deviate from the circumference of a perfect circle. This problem arises in a variety of applications in signal processing ranging from breast imaging to sensor network localization. We introduce a novel method of calibration/localization based on the time-of-flight (ToF) measurements between sensors when the enclosed medium is homogeneous. In the presence of all the pairwise ToFs, one can easily estimate the sensor positions using multi-dimensional scaling (MDS) method. In practice however, due to the transitional behaviour of the sensors and the beam form of the transducers, the ToF measurements for close-by sensors are unavailable. Further, random malfunctioning of the sensors leads to random missing ToF measurements. On top of the missing entries, in practice an unknown time delay is also added to the measurements. In this work, we incorporate the fact that a matrix defined from all the ToF measurements is of rank at most four. In order to estimate the missing ToFs, we apply a state-of-the-art low-rank matrix completion algorithm, OPTSPACE . To find the correct positions of the sensors (our ultimate goal) we then apply MDS. We show analytic bounds on the overall error of the whole process in the presence of noise and hence deduce its robustness. Finally, we confirm the functionality of our method in practice by simulations mimicking the measurements of a circular ultrasound tomography device.

==> Figures/C_inc_AssumedPositions.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{C_inc_AssumedPositions}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           30-Nov-2010 09:38:23
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-0.1}%
\psfrag{x02}[t][t]{-0.05}%
\psfrag{x03}[t][t]{0}%
\psfrag{x04}[t][t]{0.05}%
\psfrag{x05}[t][t]{0.1}%
%
% yticklabels:
\psfrag{v01}[l][l]{1200}%
\psfrag{v02}[l][l]{1500}%
\psfrag{v03}[l][l]{1800}%
\psfrag{v04}[r][r]{-0.1}%
\psfrag{v05}[r][r]{-0.05}%
\psfrag{v06}[r][r]{0}%
\psfrag{v07}[r][r]{0.05}%
\psfrag{v08}[r][r]{0.1}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{C_inc_AssumedPositions.eps}}%
\end{psfrags}%
%
% End C_inc_AssumedPositions.tex


==> Figures/C_inc_with_t0_AssumedPositions.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{C_inc_with_t0_AssumedPositions}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           30-Nov-2010 09:37:58
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-0.1}%
\psfrag{x02}[t][t]{-0.05}%
\psfrag{x03}[t][t]{0}%
\psfrag{x04}[t][t]{0.05}%
\psfrag{x05}[t][t]{0.1}%
%
% yticklabels:
\psfrag{v01}[l][l]{1200}%
\psfrag{v02}[l][l]{1500}%
\psfrag{v03}[l][l]{1800}%
\psfrag{v04}[r][r]{-0.1}%
\psfrag{v05}[r][r]{-0.05}%
\psfrag{v06}[r][r]{0}%
\psfrag{v07}[r][r]{0.05}%
\psfrag{v08}[r][r]{0.1}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{C_inc_with_t0_AssumedPositions.eps}}%
\end{psfrags}%
%
% End C_inc_with_t0_AssumedPositions.tex


==> Figures/C_orig_AssumedPositions.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{C_orig_AssumedPositions}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           30-Nov-2010 09:38:50
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-0.1}%
\psfrag{x02}[t][t]{-0.05}%
\psfrag{x03}[t][t]{0}%
\psfrag{x04}[t][t]{0.05}%
\psfrag{x05}[t][t]{0.1}%
%
% yticklabels:
\psfrag{v01}[l][l]{1200}%
\psfrag{v02}[l][l]{1500}%
\psfrag{v03}[l][l]{1800}%
\psfrag{v04}[r][r]{-0.1}%
\psfrag{v05}[r][r]{-0.05}%
\psfrag{v06}[r][r]{0}%
\psfrag{v07}[r][r]{0.05}%
\psfrag{v08}[r][r]{0.1}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{C_orig_AssumedPositions.eps}}%
\end{psfrags}%
%
% End C_orig_AssumedPositions.tex


==> Figures/C_orig_FoundPositions.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{C_orig_FoundPositions}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           07-Dec-2010 16:30:16
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-0.1}%
\psfrag{x02}[t][t]{-0.05}%
\psfrag{x03}[t][t]{0}%
\psfrag{x04}[t][t]{0.05}%
\psfrag{x05}[t][t]{0.1}%
%
% yticklabels:
\psfrag{v01}[l][l]{1490}%
\psfrag{v02}[l][l]{1500}%
\psfrag{v03}[l][l]{1510}%
\psfrag{v04}[r][r]{-0.1}%
\psfrag{v05}[r][r]{-0.05}%
\psfrag{v06}[r][r]{0}%
\psfrag{v07}[r][r]{0.05}%
\psfrag{v08}[r][r]{0.1}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{C_orig_FoundPositions.eps}}%
\end{psfrags}%
%
% End C_orig_FoundPositions.tex

